Observation of spin-splitter torque in collinear antiferromagnetic RuO$_2$

The spin-splitter effect is theoretically predicted to generate an unconventional spin current with $\mathit{x}$- and $\mathit{z}$- spin polarization via the spin-split band in antiferromagnets. The generated torque, namely spin-splitter torque, is effective for the manipulation of magnetization in an adjacent magnetic layer without an external magnetic field for spintronic devices such as MRAM. Here, we study the generation of torque in collinear antiferromagnetic RuO$_2$ with (100), (101), and (001) crystal planes. Next we find all $\mathit{x}$-, $\mathit{y}$-, and $\mathit{z}$-polarized spin currents depending on the N\'{e}el vector direction in RuO$_2$(101). For RuO$_2$(100) and (001), only $\mathit{y}$-polarized spin current was present, which is independent of the N\'{e}el vector. Using the $\mathit{z}$-polarized spin currents, we demonstrate field-free switching of the perpendicular magnetized ferromagnet at room temperature. The spin-splitter torque generated from RuO$_2$ is verified to be useful for the switching phenomenon and paves the way for a further understanding of the detailed mechanism of the spin-splitter effect and for developing antiferromagnetic spin-orbitronics.

==> tex/01_model.tex <==
\section{TEST}


==> tex/11_data_ava.tex <==
\section*{Data Availability}
The data that support the findings of this study are available from the corresponding author upon reasonable request.
